Dissecting CXL Memory Performance at Scale: Analysis, Modeling, and Optimization

We present SupMario, a characterization framework designed to thoroughly analyze, model, and optimize CXL memory performance. SupMario is based on extensive evaluation of 265 workloads spanning 4 real CXL devices within 7 memory latency configurations across 4 processor platforms. SupMario uncovers many key insights, including detailed workload performance at sub-us memory latencies (140-410 ns), CXL tail latencies, CPU tolerance to CXL latencies, CXL performance root-cause analysis and precise performance prediction models. In particular, SupMario performance models rely solely on 12 CPU performance counters and accurately fit over 99% and 91%-94% workloads with a 10% misprediction target for NUMA and CXL memory, respectively. We demonstrate the practical utility of SupMario characterization findings, models, and insights by applying them to popular CXL memory management schemes, such as page interleaving and tiering policies, to identify system inefficiencies during runtime. We introduce a novel ``bestshot'' page interleaving policy and a regulated page tiering policy (Alto) tailored for memory bandwidth- and latency-sensitive workloads. In bandwidth bound scenarios, our ``best-shot'' interleaving, guided by our novel performance prediction model, achieves close-to optimal scenarios by exploiting the aggregate system and CXL/NUMA memory bandwidth. For latency sensitive workloads, Alto, driven by our key insight of utilizing ``amortized'' memory latency to regulate unnecessary page migrations, achieves up to 177% improvement over state-of-the-art memory tiering systems like TPP, as demonstrated through extensive evaluation with 8 real-world applications.

==> Makefile <==
#-------------------------------------------------------------------------------
#
# Makefile to compile the paper
# Usage:
#     - ``make h``: compile the tex files into "main.pdf"
#     - ``make p``: compile and open "main.pdf" using ~/bin/pdfreader (wrapper
#       of evince, mpdf, zathura, etc.)
#
#-------------------------------------------------------------------------------

MAIN      = main
SRCS      = *.tex
PS        = $(MAIN).ps
PDF       = $(MAIN).pdf
DVI       = $(MAIN).dvi
TARG      = $(MAIN).done

all: texnoredo #cleanabit

h: all cleanabit # ps pdf

p: all openpdf cleanabit #ps pdf

s: openpdf

b: main.pdf
	${HOME}/bin/backup-file main.pdf

openpdf:
	${HOME}/bin/pdfreader main.pdf

diff:
	docs/diff.sh 44851a377ff7398da9ba5bdcea1d47facee077ee

texwithredo:
	pdflatex main.tex
	bibtex -min-crossrefs=1000 main
	pdflatex main.tex
	pdflatex main.tex

texnoredo:
	pdflatex main.tex
	bibtex -min-crossrefs=1000 main
	pdflatex main.tex
	pdflatex main.tex

e:
	pdflatex extended_abstract.tex
	bibtex -min-crossrefs=100 extended_abstract
	pdflatex extended_abstract.tex
	pdflatex extended_abstract.tex

texnobib:
	pdflatex main.tex

$(MAIN).bbl: $(MAIN).aux
	bibtex -min-crossrefs=200 $(MAIN)
	./redo-bib.csh $(MAIN)

$(MAIN).aux: $(MAIN).tex
	latex $(MAIN)

ps: $(DVI)
	dvips -o $(PS) $(MAIN)

pdf: $(PS)
	ps2pdf14 $(PS)

clean:
	rm -vf *.ps  main.pdf *.dvi *.aux *.log \
	*.bbl *.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png *.toc

cleanabit:
	rm -vf *~ *.ps  *.aux *.log \
	*.bbl *.blg *.out *.brf *.4*  \
	*.css *.idv *.lg *.tmp *.xref *.png *.toc


==> bib.tex <==
%\newpage
%\setcounter{page}{1}
%\thispagestyle{empty}

%\singlespacing
\setlength{\bibsep}{2pt plus 0.1ex}
%\raggedright
{\small
   \bibliographystyle{plain}
   \bibliography{bib-p-mario.tex.bib,B/confs}
   %\bibliography{main}
}



==> des.tex <==
\section{Design}
\label{sec-des}

This is our design section.


==> eval.tex <==
\section{Evaluation}
\label{sec-eval}

This is our evaluation section.


==> fig-latbw.tex <==

\begin{figure}[t!]
%\begin{floatingfigure}[r]{2.2in}
%\hspace*{-20pt}
\centerline{
\includegraphics[width=3.in]{F/new/lat-bw/eps/one-latbw.pdf}
}
%
\vminfive
%
\mycaption{fig:latbw}{CXL device loaded latency vs. bandwith}{CXL
latency increases when device bandwidth is close to saturation with a
steeper changing rate vs. local/NUMA memory.}
%
\vminten
%\end{floatingfigure}
\end{figure}



==> fig-sample.tex <==

\def \hmina {\hspace{-0.1in}}
\def \hminb {\hspace{-0.2in}}

\begin{figure}[t!]
    %\hmina
    \centering
    \includegraphics[width=0.98\columnwidth]{F/sketches/workflow-hcl}
    \mycaption{fig-workflow}{\sys control plane workflow}{ {\bf A)}~The
        VM scheduler uses ML-based predictions that identify
        latency-sensitive VMs and their likely amount of untouched
        memory to decide on VM placement (see Figure~\ref{fig-premodels}).
        {\bf B)} The monitoring pipeline reconfigures VMs if quality-of-service
        (QoS) not met.}
\end{figure}


==> fig-sldwn.tex <==

\begin{figure}[h]
%\begin{floatingfigure}[r]{2.2in}
%\hspace*{-20pt}
\centerline{
\includegraphics[width=3.in]{F/new/sldwn/sldwn-cdf.pdf}
}
%
\mycaption{fig-arch}{Workload slowdown CDF under CXL}{}
%
%\end{floatingfigure}
\end{figure}



==> fig-slowdown-cdf.tex <==

\begin{floatingfigure}[r]{1.3in}
    \centering
    \vspace{-32pt}
    \includegraphics[width=1.3in]{F/new/brk-acc/eps/brk-ac.pdf}
    \vspace{-4mm}
    \mycaption{fig:brk-acc}{Accuracy}{}
    \vspace{-2mm}
\end{floatingfigure}


==> fig-w-all.tex <==

\begin{figure}[t!]
%\begin{floatingfigure}[r]{2.2in}
%\hspace*{-20pt}
\centerline{
\includegraphics[width=.55\columnwidth]{F/new/sldwn/eps/spr-vs-emr-cpu2017.pdf}
\includegraphics[width=.55\columnwidth]{F/new/sldwn/eps/sldwn-cdf.pdf}
}
%
\mycaption{fig:allcdf}{Slowdown cdf}{}
%
%\end{floatingfigure}
\end{figure}



==> tab-findings.tex <==

%\newpage

\setlength{\tabcolsep}{4pt}

%Workload specific findings: performance of modern high performance I/O
%devices (\eg, NVMe SSDs) will be significantly affected; VoltDB is
%experience much less performance impact than Redis; Spark workload
%(usually with the highest observable DRAM traffic) are not severely
%impacted as graph processing workloads. \\ \hline

\newcounter{fc}
\setcounter{fc}{0}
\newcommand{\myf}{{\refstepcounter{fc}\arraybackslash\thefc\arraybackslash}}

\vminfive
\begin{table*}[th!]
\begin{center}
\mycaption{tab:findings}{Summary of findings}{}
\vminfive
\small
%\footnotesize
%\scriptsize
\rowcolors{2}{gray!20}{white} % Define row colors: alternate rows in gray!10 and white
\begin{tabular}{cp{8.5cm}p{7cm}}
\hline
& {\bf Key Findings and Observations} & {\bf Implications / Root Causes} \\
\hline
1 & CXL-DRAM have unstable and variable memory access latency. & Real-world applications will be affected by unstable memory access latency, resulting in less predictability for their performance on CXL-DRAM. \\

2 & Not all CXL deivices are created equal, each carrying unique performance characteristics. Different kinds of devices have different types of tail latency. & Tail latency should be used as a metric to evaluate CXL devices. CXL controllers may need further optimizations. \\

3 & Longer CXL latencies correspond to worse bandwidth, which has a more pronounced impact on bandwidth-bounded workloads compared to latency-bounded workloads, due to the combined effects of longer latency and limited bandwidth. & Software approaches are needed for bandwidth-bound workloads to effectively utilize the combined bandwidth of local and CXL memory. \\

4 & CXL slowdown can be attributed to different hardware components: DRAM load, cache, and store, corresponding to demand reads, prefetching, and RFO. & CXL impacts various stages of the CPU pipeline, necessitating careful examination based on workload memory access patterns. \\

5 & Bandwidth/LLC-miss-rate is independent of CXL performance while stall-based metric {\it perfectly} captures it & Need better methods to analyze/predict CXL-caused slowdowns \\

6 & CXL slowdown can be predicted accurately with a linear model that cleverly combines a little more than ten CPU PMU counters in an explainable and reasonable way. & Workload performance under CXL can be predicted. Our CXL performance prediction model can enable many potential use cases, such as serving as a drop-in replacement for pool memory predictor to guide CXL memory allocation decisions for VMs in the cloud. \\

7 & Cache slowdown is mainly caused by prefetching, which can be verified by both disabling prefetchers and reasoning with CPU counters. & CPU prefetcher efficiency is negatively impacted by CXL’s longer access latency, causing performance slowdowns at the cache level (e.g., LFB). \\

8 & Non-bandwidth-bound workloads typically cannot benefit from NUMA page interleaving. Even for bandwidth-bound workloads, various slowdowns (and occasional speedups) were observed across different interleaving ratio settings, reflecting the combined impact of CXL latency and bandwidth. Various bandwidth-bound workloads have different optimal interleaving ratios, potentially outperforming local DRAM performance. & When deploying bandwidth-bound workloads on CXL, there is a need to: 1. Predict whether a workload can benefit from interleaving (otherwise refer to a tiering policy). 2. Predict the best interleaving ratio in one run. 3. Predict potential performance gains. Bandwidth-bound workloads should use interleaving to improve performance. We suggest users adopt our best-shot interleaving policy to deploy workloads on CXL without hassle. \\

% 3 & Different phases of workload see varying slowdowns from dynamically changing components (\eg, {Store}, {Cache}) & Dynamic memory access pattern gives dynamic and complicated slowdown during runtime \\

% 4 & Stalled cycles can be monitored and showed almost linear-correlation with CXL slowdowns  & A ``stall''-based linear model can help accurately predict CXL slowdowns for memory optimizations \\

%& Mixing with 80\% local DRAM ensured good perfornamce for XX-YY\% of workloads -- but tail remains. & A static split between local and CXL DRAM is not sufficient for various types of VMs and workloads. \\

% 5 & Interleaving local/CXL memory does not work consistencly, hurting performance for some while improving it for others & OS-level memory management scheme needs to be revisited for CXL \\

% 6 & Different phases of workload see varying slowdowns from dynamically changing components (\eg, {Store}, {Cache}) & The future load-store I/O stack needs to be able to capture and adapt to workload dynamism \\

9 & Memory parallelism could alleviate CXL performance slowdown  & High parallel memory accesses will not experience significant slowdowns compared to other memory access patterns.  \\

\hline

%& TMA works better than ML and 20\% of workloads can safely be placed entirely into CXL pool & \\
%& ML works better than static for frigid memory, and we can safely predict 20\% frigid memory on average, 80\% local memory & \\
%& Stranding vs pool size, for different models. & Small pool size is enough and our prediction models make a big difference (\eg, vs. static mixing) \\
\end{tabular}
\end{center}
\label{tbl-finding}
%\vmintwenty
%\vminfive

\end{table*}

\vfive



==> tab-model-error.tex <==

% https://docs.google.com/spreadsheets/d/1BwEdu_yQtWXcxO2DB1cyJbjsovevH1JctAz8HwZfC1A/edit?gid=824155242#gid=824155242

\setlength{\tabcolsep}{2pt}

% ------------------------------------------- table sample
\begin{floatingfigure}[r]{2in}
\begin{center}
{\small
%---------------------------------
\begin{tabular}{c|ccc}
%{\bf } & \multicolumn{2}{c}{Col1}
%       & \multicolumn{2}{c}{Col2} \\
       &   \znuma   &   \cxla   &  \cxlb   \\
\hline
Pearson       &   0.95   &   0.85   &   0.84     \\
\hline
5\%       &   3.1\%   &   31.3\%   &   43.3\%     \\
\hline
 10\%      &   1.25\%   &   12.5\%   &   15.3\%    \\
 15\%      &   0\%     &    4.4\%    &   7.4\% \\
 20\%      &   0\%    &     1.3\%    &   3.7\% \\
\end{tabular}
}
%---------------------------------
\end{center}
\vminfifteen
\mycaption{tab:pred-err}{Mispredictions}{Prediction model of \znuma is most robust.}
\end{floatingfigure}

